Mask-Adapter: The Devil is in the Masks for Open-Vocabulary Segmentation

Recent open-vocabulary segmentation methods adopt mask generators to predict segmentation masks and leverage pre-trained vision-language models, e.g., CLIP, to classify these masks via mask pooling. Although these approaches show promising results, it is counterintuitive that accurate masks often fail to yield accurate classification results through pooling CLIP image embeddings within the mask regions. In this paper, we reveal the performance limitations of mask pooling and introduce Mask-Adapter, a simple yet effective method to address these challenges in open-vocabulary segmentation. Compared to directly using proposal masks, our proposed Mask-Adapter extracts semantic activation maps from proposal masks, providing richer contextual information and ensuring alignment between masks and CLIP. Additionally, we propose a mask consistency loss that encourages proposal masks with similar IoUs to obtain similar CLIP embeddings to enhance models' robustness to varying predicted masks. Mask-Adapter integrates seamlessly into open-vocabulary segmentation methods based on mask pooling in a plug-and-play manner, delivering more accurate classification results. Extensive experiments across several zero-shot benchmarks demonstrate significant performance gains for the proposed Mask-Adapter on several well-established methods. Notably, Mask-Adapter also extends effectively to SAM and achieves impressive results on several open-vocabulary segmentation datasets. Code and models are available at https://github.com/hustvl/MaskAdapter.

==> sec/0_abstract.tex <==
\begin{abstract}
Recent open-vocabulary segmentation methods adopt mask generators to predict segmentation masks and leverage pre-trained vision-language models, \eg, CLIP, to classify these masks via mask pooling.
Although these approaches show promising results, 
% using proposal masks and mask pooling to 
it is counterintuitive that accurate masks often fail to yield accurate classification results through pooling CLIP image embeddings within the mask regions.
% , which can be attributed to the misalignment between masks and CLIP,
In this paper, we reveal the performance limitations of mask pooling and introduce \textbf{\name{}}, a simple yet effective method to address these challenges in open-vocabulary segmentation.
Compared to directly using proposal masks, our proposed \name{} extracts \textit{semantic activation maps} from proposal masks, providing richer contextual information and ensuring alignment between masks and CLIP.
Additionally, we propose a \textit{mask consistency loss} that encourages proposal masks with similar IoUs to obtain similar CLIP embeddings to enhance models' robustness to varying predicted masks.
\name{} integrates seamlessly into open-vocabulary segmentation methods based on mask pooling in a plug-and-play manner, delivering more accurate classification results. Extensive experiments across several zero-shot benchmarks demonstrate significant performance gains for the proposed \name{} on several well-established methods.
Notably, \name{} also extends effectively to SAM and achieves impressive results on several open-vocabulary segmentation datasets.
Code and models are available at \url{https://github.com/hustvl/MaskAdapter}.

\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{sec/figures/intro_figure.pdf}
    \vspace{-20pt}
    \caption{\textbf{Upper bound analysis of mask embedding extraction methods.} Using ADE20K ground-truth masks as input, we evaluate the upper bound of different extraction methods. While mask cropping and mask pooling show limited performance with ground-truth masks, our Mask-Adapter significantly enhances the upper bound for open-vocabulary segmentation.}
    \label{fig:intro}
    \vspace{-10pt}
\end{figure}


Image segmentation, which aims to assign each pixel a label from a predefined set of categories, has seen significant advancements.
Despite the success of numerous image segmentation approaches~\cite{cheng2022masked,chen2018encoder,xie2021segformer,wang2020deep,zheng2021rethinking,strudel2021segmenter}, these approaches cannot segment categories unseen during training, limiting their applicability in open-world scenarios.
Open-vocabulary segmentation (OVS) has expanded traditional image segmentation from fixed-set to open-set, enabling the segmentation of categories not appeared in the training set.
In contrast to fixed-category segmentation, open-vocabulary segmentation not only supports open-set segmentation but also enables challenging segmentation based on arbitrary text inputs, \eg, categories and descriptions.

\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{sec/figures/intro_figure_comp.pdf}
    \vspace{-15pt}
    \caption{\textbf{Comparison of mask embedding extraction methods.} (a) \textbf{Mask Cropping}: cropping the segmented region from the image and feeding it into CLIP to extract mask embeddings. (b) \textbf{Mask Pooling}: aggregating region features with the proposal masks. (c) \textbf{Mask-Adapter}: the proposal masks and CLIP features are passed through Mask-Adapter to extract semantic activation maps, which are then used to construct mask embeddings by aggregating CLIP features based on these highlighted regions and contextual information.}
    \label{fig:com_methods}
\end{figure*}

Recent research tackles open-vocabulary segmentation by leveraging pre-trained vision-language models, \eg, CLIP~\cite{radford2021learning} and ALIGN~\cite{jia2021scaling}, which are pre-trained on large-scale image-text pairs and have strong zero-shot recognition capabilities.
Notably, several works~\cite{xu2022simple,ding2022decoupling,liang2023open,han2023open,yu2023convolutions,jiao2024collaborative,shan2024open,xu2024generalization}, such as SimpleBaseline~\cite{xu2022simple} FC-CLIP~\cite{yu2023convolutions}, follow a \textit{segment-then-recognize} paradigm for open-vocabulary segmentation, which adopts mask generators to predict proposal masks from images and then classify the proposal masks by transferring the zero-shot recognition capability from the frozen CLIP.
Recognizing segmentation masks is primarily achieved by extracting mask embeddings through the CLIP visual encoder and matching them with text embeddings.
Specifically, the mask embeddings can be obtained in two ways: (1) \textit{mask cropping}~\cite{xu2022simple,ding2022decoupling,liang2023open}: cropping the segmented region from the image and using CLIP to extract image embeddings; (2) \textit{mask pooling}~\cite{ghiasi2022scaling,yu2023convolutions,jiao2024collaborative,shan2024open,xu2024generalization}: directly aggregating the features of the region using mask pooling~\cite{ghiasi2022scaling} with the proposal masks through dot-product, which is more efficient than mask cropping and can be end-to-end optimized.
% New Add %
However, the upper bound of these two methods for open-vocabulary segmentation is inherently limited, as shown in Fig.~\ref{fig:intro}. The mask cropping method (Fig.~\ref{fig:com_methods} (a)) fails to account for the substantial differences between the masked image and the natural images used during CLIP~\cite{radford2021learning} pre-training, as mentioned in~\cite{liang2023open}. Meanwhile, the mask pooling method (Fig.~\ref{fig:com_methods} (b)) fails to capture semantic details and contextual information during feature aggregation, limiting its upper bound.

In this paper, we propose a simple yet effective method to address the bottlenecks in open-vocabulary segmentation. Instead of directly using predicted masks and mask pooling (or mask cropping) to extract mask embeddings, we introduce a \textit{\name{}} (Fig.~\ref{fig:com_methods} (c)) to extract \textit{semantic activation maps} from proposal masks and CLIP features. 
Mask embeddings are aggregated based on both semantic and contextual information and subsequently matched with text embeddings for mask recognition. Fig.~\ref{fig:com_methods} compares mask cropping, mask pooling, and Mask-Adapter methods. In contrast to previous approaches, Mask-Adapter offers several key advantages: (1) rather than neglecting the background, it aggregates mask embeddings across the entire image, incorporating contextual information to enrich the feature representation; (2) unlike mask pooling, which only conveys the positional information of target regions, semantic activation maps selectively highlights informative regions relevant to recognition, while suppressing less informative areas, thus enhancing feature discriminability; (3) our method preserves the generalization capabilities of CLIP during training while concurrently improving mask recognition performance. Furthermore, we introduce a mask consistency loss to enforce similar proposal masks to obtain similar CLIP mask embeddings, thereby improving robustness to variations in predicted masks. To further mitigate overfitting, we replace the Hungarian matcher with an IoU-based matcher, enabling the model to train on a broader range of proposal masks.
In addition, we propose a mixed-mask training strategy that enhances the robustness of the Mask Adapter and improves its performance on open-vocabulary segmentation tasks.
% Our training procedure follows a two-stage approach: first, a ground-truth mask warmup phase is employed, followed by mixed-mask training. This training strategy enhances Mask-Adapter’s robustness and improves its performance on open-vocabulary segmentation tasks.

The main contributions of this paper can be summarized as follows:
\begin{itemize}
    \item We introduce the Mask-Adapter, which addresses critical bottlenecks, \ie, misalignment between pre-trained CLIP and segmentation masks, in open-vocabulary segmentation and can be integrated seamlessly into mask pooling-based methods in a plug-and-play manner, delivering more accurate classification results.
    \item We introduce a mask consistency loss and present an IoU-based matcher to reduce overfitting and improve the robustness of \name{} along with a mixed-mask training strategy.
    \item We integrate the proposed Mask-Adapter into established open-vocabulary segmentation frameworks, demonstrating substantial performance improvements and achieving state-of-the-art results on datasets such as ADE20K and Pascal-Context. Furthermore, the Mask-Adapter effectively extends to SAM without training, achieving impressive results across multiple open-vocabulary segmentation benchmarks.
\end{itemize}



% In this paper, we propose a simple yet effective method aiming to tackle the bottlenecks in open-vocabulary segmentation. To address these issues, we introduce a \textit{Mask Adapter} approach that generates a semantic activation map by combining masks with CLIP features, which highlights informative regions for each mask while also providing valuable contextual cues. Mask embeddings are then constructed by aggregating CLIP features based on these highlighted regions and contextual information, and the similarity between mask embeddings and text embeddings is calculated to produce predicted probabilities.The Mask Adapter offers several advantages over existing methods: (1) It aggregates mask features across the entire image rather than ignoring the background, thereby incorporating richer contextual information. (2) Unlike mask-pooling, which only conveys the positional information of targets, the semantic activation map selectively highlights regions conducive to recognition while suppressing less informative areas, enhancing feature discriminability. (3) Our approach preserves CLIP’s inherent generalization abilities during training while enhancing mask recognition. To improve matching, we employ an IoU-based matcher rather than a Hungarian matcher, capturing a wider variety of masks. Additionally, we introduce a mask cosine loss to enforce consistency within mask embeddings, improving recognition of unseen classes.Our training approach employs a two-stage process, beginning with a ground-truth warmup phase and followed by mixed-mask training. This setup ensures both training stability and strong generalization performance, making the Mask Adapter a robust solution for open-vocabulary segmentation.





% Recently, 

% Open-vocabulary segmentation~\cite{} extends image segmentation to 
% Image segmentation, as the most fundamental task of computer vision, aims to assign a semantic label to each pixel in an image.
% Open-vocabulary segmentation~\cite{} extends image segmentation 
% Image segmentation aims to assign a semantic label to each pixel in an image. With advances in attention mechanisms \cite{vaswani2017attention} and convolutional neural networks, recent works \cite{cheng2022masked,chen2018encoder,xie2021segformer,wang2020deep} have achieved remarkable success on large-scale benchmarks such as ADE20K~\cite{zhou2019semantic}. However, these methods are limited to segmenting only the predefined categories seen during training. In contrast, \textit{open-vocabulary segmentation} enables segmentation based on arbitrary textual descriptions, aligning more closely with human perception and cognitive processes. Despite its promising potential, developing open-vocabulary segmentation methods that match the performance of supervised models while generalizing effectively across categories remains a significant challenge.

% Pretraining on large-scale internet image-text pairs, CLIP\cite{radford2021learning} bridges the gap between visual and textual modalities and demonstrates impressive open-vocabulary recognition capabilities. 
% Transferring CLIP's zero-shot recognition capability to open-vocabulary segmentation has thus become a mainstream approach. Current methods generally consist of two stages: first, a mask generator produces class-agnostic masks, and then CLIP is used to perform mask classification. However, mask classification has become a bottleneck in open-vocabulary segmentation, limiting the performance of current methods. Some methods \cite{xu2022simple,ding2022decoupling,liang2023open} attempt to classify masks by cropping and masking image regions, then feeding them into CLIP for classification. However, these methods disregard the considerable differences between the masked images and the natural images used during pretraining. Moreover, segmentation tasks typically require high resolution, which conflicts with CLIP’s low-resolution design, resulting in suboptimal classification performance. Recent approaches\cite{ghiasi2022scaling,yu2023convolutions,jiao2024collaborative}  have adopted Mask Pooling to capture features within mask regions, achieving promising results. However, this method only provides positional information and lacks semantic context. Moreover, it completely disregards the regions outside the object, leading to a lack of contextual information. These limitations result in low mask classification accuracy in open-vocabulary segmentation.




==> sec/2_related_works.tex <==
\section{Related Work}
\label{sec:formatting}

\subsection{Open-Vocabulary Segmentation}
Open-vocabulary segmentation aims to segment images based on arbitrary textual descriptions rather than predefined classes, primarily categorizing into two types: per-pixel classification~\cite{li2022language,cho2024cat,xie2024sed} and mask classification~\cite{ghiasi2022scaling,xu2022simple,ding2022decoupling,han2023open,liang2023open,xu2023open,yu2023convolutions,jiao2024collaborative}. OpenSeg~\cite{ghiasi2022scaling} first employs mask pooling method to aggregate region features for mask classification.
SimpleBaseline~\cite{xu2022simple} and Zegformer~\cite{ding2022decoupling} propose two-stage frameworks which generate class-agnostic masks and feed the masked image into CLIP for classification.
Per-pixel methods, \eg, CAT-Seg~\cite{cho2024cat} and SED~\cite{xie2024sed}, adopt cost aggregation to refine the pixel-text cost volume and predict per-pixel classification outputs. PrimitiveNet~\cite{liu2024primitivenet} decomposes complex language constraints into simple primitives and employs cross-primitive and language-primitive attention mechanisms to enhance referring segmentation performance. SAN~\cite{xu2023san} attaches an adapter to CLIP, enabling mask proposal generation and recognition.
FC-CLIP~\cite{yu2023convolutions} utilizes CLIP as a shared backbone for both mask generation and mask classification. However, both mask cropping and mask pooling approaches used in previous mask classification methods to obtain mask embeddings exhibit a limited upper bound performance, as illustrated in Fig.~\ref{fig:intro}.

Several works~\cite{liang2023open, xie2024sed} point out that the bottleneck of open-vocabulary segmentation lies in CLIP-based mask classification. 
OVSeg~\cite{liang2023open} observes the significant gap between masked images and natural images when using CLIP and addresses it by adapting CLIP with masked image-category pairs. 
MaskCLIP~\cite{ding2022open} and MasQCLIP~\cite{xu2023masqclip} adopt masked attention instead of mask cropping for mask classification. MAFT~\cite{jiao2023learning} finetunes the CLIP image encoder while employing a self-distillation loss to prevent catastrophic forgetting, and MAFTP~\cite{jiao2024collaborative} further introduces content-dependent transfer to fine-tune the text representations.
Deop~\cite{han2023open} decouples mask generation and classification and employs a heatmap-based pooling method instead of mask pooling, but its open-vocabulary segmentation performance remains relatively weak. In contrast, our proposed Mask-Adapter extracts \textit{semantic activation maps} from proposal masks, providing richer contextual information and ensuring better alignment between masks and CLIP. Compared to Deop, our method differs in the following key aspects: (1) our Mask-Adapter is a standalone module that can be integrated seamlessly into open-vocabulary segmentation methods and SAM model; (2) the structure our Mask-Adapter differs from the heatmap decoder in Deop. Specifically, our Mask-Adapter extracts semantic activation maps from proposal masks, rather than generating heatmaps based on image features and masks, thereby capturing richer contextual and semantic information; (3) during mask-text alighment training, we introduce a mask consistency loss and employ an IoU-based matcher to enhance the model's robustness to varying predicted masks. Furthermore, we employ a two-stage training strategy, incorporating ground-truth warmup and mixed-mask training, to stabilize training and preserve generalization. Additionally, by integrating Mask-Adapter into several well-established methods, we obtain significant improvements and achieve new state-of-the-art results across multiple datasets.









%-------------------------------------------------------------------------
\subsection{Adaptation for Vision-Language Models}
Recent advancements in vision-language pre-training models,  \eg, CLIP~\cite{radford2021learning} and ALIGN~\cite{jia2021scaling}, have demonstrated strong open-vocabulary recognition capabilities. To further enhance CLIP's performance, various adaptation strategies have been proposed. Notably, prompt tuning methods like CoOp~\citep{zhou2022learning} and CoCoOp~\citep{zhou2022conditional} integrate learnable prompts, replacing handcrafted text prompts to improve domain-specific adaptation. Feature-based methods, such as CLIP-Adapter~\citep{gao2024clip} and Tip-Adapter~\citep{zhang2021tip}, introduce lightweight adapters. CLIP-Adapter fine-tunes features through a bottleneck layer, combining learned and pre-trained features, while Tip-Adapter enhances few-shot learning with minimal fine-tuning via a cache model. Despite achieving good results in image classification, CLIP and these adaptations still struggle with dense prediction tasks like open-vocabulary object detection and segmentation.

To address CLIP’s limitations in dense prediction tasks, several methods have been proposed. CLIPSelf~\citep{wu2023clipself} and SILC~\citep{naeem2023silc} leverage self-distillation to align global and local features. Furthermore, Yolo-World~\citep{cheng2024yolo} integrates the CLIP text encoder with a lightweight detector for open-vocabulary object detection, while EVF-SAM~\citep{zhang2024evf} utilizes early vision-language fusion to enable text-prompted SAM for referring expression segmentation tasks. Other approaches, such as MaskCLIP~\citep{zhou2022extract}, CLIPSurgery~\citep{li2023clip}, SCLIP~\citep{wang2023sclip}, and GEM~\citep{bousselham2024grounding}, modify CLIP's attention structure to enhance its performance on dense prediction tasks. Furthermore, GBA~\citep{xu2024generalization} introduces learnable adapters to boost CLIP's generalization in open-vocabulary segmentation, while PixelCLIP~\citep{shin2024towards} improves CLIP's fine-grained pixel representation by leveraging vision foundation models (e.g., DINO~\citep{caron2021emerging}, SAM~\citep{kirillov2023segment}) and unlabeled masks. Despite these advancements, CLIP continues to underperform in open-vocabulary region recognition tasks.

%-------------------------------------------------------------------------



==> sec/3_method.tex <==


\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{sec/figures/main.pdf}
    \vspace{-15pt}
    \caption{\textbf{Overview of \name.} (a) Mask-Adapter for Open-Vocabulary Segmentation. Mask-Adapter can be seamlessly integrated into open-vocabulary segmentation methods based on mask pooling. Mask-Adapter extracts semantic activation maps from CLIP features and proposal masks. Mask embeddings are aggregated according to semantic activation maps, which provide richer contextual and semantic information. The aggregated mask embeddings are then matched with text embeddings to perform mask classification. During training, only the Mask-Adapter is trainable. (b) Details of the Mask-Adapter. After patchifying the masks, masks and CLIP features are fused and processed through ConvNeXt blocks, ultimately outputting the semantic activation maps through a predictor.}
    \label{fig:main_arch}
    \vspace{-10pt}
\end{figure*}


\section{Approach}
% In this section, we mainly tackle the bottlenecks in open-vocabulary segmentation by presenting \textit{Mask-Adapter} to boost the accuracy of mask classification.

% In this section, we define mask classification as the primary bottleneck in open-vocabulary segmentation and revisit existing zero-shot mask classification methods to clarify their limitations. Inspired by \cite{han2023open,cheng2022sparse}, we propose our \textit{Mask-Adapter} method, which substantially improves mask classification accuracy in the open-vocabulary segmentation framework while preserving CLIP’s original generalization ability.

% \subsection{Recognize Any Mask}
% mask -> CLIP -> mask-pooling -> recognize
\subsection{Problem Definition}
Open-vocabulary segmentation aims to segment images based on arbitrary textual descriptions, rather than a fixed set of predefined classes. This task involves training the model on a set of seen categories $\mathbf{C}_{\text{seen}}$ and evaluating its performance on both the seen categories $\mathbf{C}_{\text{seen}}$ and the unseen categories $\mathbf{C}_{\text{unseen}}$.
Existing open-vocabulary segmentation methods~\cite{xu2022simple,ding2022decoupling,liang2023open,jiao2024collaborative,yu2023convolutions} are composed of a class-agnostic mask generator and a mask classifier.
The mask generator, \eg, Mask2Former~\cite{cheng2022masked}, produces class-agnostic masks $M_p \in \mathbb{R}^{N \times H \times W} $, and the mask classifier categorizes these masks according to text descriptions.

Given \( N \) class-agnostic masks \( M_p \in \mathbb{R}^{N \times H \times W} \) generated by the mask generator, the initial approach~\cite{xu2022simple,ding2022decoupling} utilizes \textit{mask cropping} (Fig.~\ref{fig:com_methods} (a)), which crops the segmented regions from the image and uses CLIP to extract image embeddings, as shown in the following Eq.~\ref{maskcropping}:
\begin{equation}
    \mathbf{E}_{\text{mask}} = \text{CLIP}(\text{crop}(M_p, \mathcal{I})) \in \mathbb{R}^{N \times C}.
    \label{maskcropping}
\end{equation}
The mask embeddings are then matched with text embeddings to recognize the segmentation masks. However, the gap between masked and natural images limits the upper bound of this method for open-vocabulary segmentation.

Methods such as \cite{ghiasi2022scaling,yu2023convolutions,jiao2024collaborative} employ a \textit{mask pooling} approach (Fig.~\ref{fig:com_methods} (b)) to obtain the mask embedding. In this method, CLIP features are aggregated via mask pooling with the proposal masks, providing greater efficiency than mask cropping, as shown in the following Eq.~\ref{maskpooling}:
\begin{equation}
    \label{maskpooling}
    \mathbf{E}_{\text{mask}} = M_p \cdot \mathcal{F}_{\text{clip}}^T.
\end{equation}
However, the mask pooling method only captures positional information of the mask region, lacking both contextual and semantic features. This limitation significantly constrains its upper bound in open-vocabulary segmentation.





% Previous studies~\cite{liang2023open, chng2024semantic} have shown that the performance bottleneck in open-vocabulary segmentation lies in the mask classification process.

% \vspace{-8pt} 
% \paragraph{Zero-shot mask classification via CLIP.}
% CLIP~\cite{radford2021learning}
% % pre-trained on large-scale image-text pair datasets 
% has demonstrated impressive open-vocabulary recognition capabilities and can be transferred for mask classification.
% % Transferring  CLIP's recognition abilities for zero-shot mask classification has become a mainstream approach. 
% Given \( N \) class-agnostic masks \( M_p \in \mathbb{R}^{N \times H \times W} \) generated by the mask generator, the initial approach~\cite{xu2022simple,ding2022decoupling} employs \textit{mask cropping} (Fig.~\ref{fig:com_methods} (a)), cropping the segmented regions from the image and using CLIP to extract image embeddings \( \mathbf{E}_{\text{mask}} = \text{CLIP}(\text{crop}(M_p, \mathcal{I})) \in \mathbb{R}^{N \times C} \). Simultaneously, the text embeddings \( \mathbf{E}_{\text{text}} \in \mathbb{R}^{T \times C} \) are generated using the CLIP Text Encoder. The classification probability for each mask is computed by calculating the similarity between the mask embeddings and the text embeddings. Specifically, as shown in Eq.~\ref{logits}, the probability for each class \( C_i \) is given by:
% \begin{equation}
%     \label{logits}
%     P(C_i | M_p) = \frac{\exp \left( \text{cosine} \left( \mathbf{E}_{\text{mask}}, \mathbf{E}_{\text{text}}^{i} \right) \big/ \delta \right)}{\sum_{j=1}^{T} \exp \left( \text{cosine} \left( \mathbf{E}_{\text{mask}}, \mathbf{E}_{\text{text}}^{j} \right) \big/ \delta \right)},
% \end{equation}
% However, this approach has several limitations. The masked image has a discrepancy from the natural images used during CLIP's pretraining, as has been observed in~\cite{liang2023open}. Furthermore, each masked image needs to be fed into CLIP for classification, resulting in substantial computational overhead. Although recent methods \cite{liang2023open} have attempted to fine-tune CLIP to improve performance, and others \cite{ding2022open,xu2023masqclip} have introduced masked attention mechanisms, these approaches still yield limited performance gains.

% Methods such as \cite{ghiasi2022scaling,yu2023convolutions,jiao2024collaborative} adopt a \textit{mask pooling} approach (Fig.~\ref{fig:com_methods} (b)) to obtain the mask embedding. In this method, CLIP features are aggregated using mask pooling with the proposal masks via dot-product, offering superior efficiency over mask cropping, as shown in Eq.~\ref{maskpooling}. Once the mask embedding is obtained, the classification probabilities are computed using Eq.~\ref{logits}.
% \begin{equation}
%     \label{maskpooling}
%     \mathbf{E}_{\text{mask}} = \text{Mask Pooling}(F_{\text{clip}}, M_p),
% \end{equation}

% Although the mask pooling approach represents mask region well and demonstrates good performance, it still falls short compared to CLIP's performance in image classification. In the mask pooling method, the mask only provides spatial location information of the target object, without incorporating its semantic features. Moreover, ignoring the background results in the loss of crucial contextual information, which limits the method's effectiveness in open-vocabulary segmentation.

\subsection{Mask-Adapter}
\paragraph{Overview.} As illustrated in Fig.~\ref{fig:main_arch}, \name{} is a simple yet remarkably effective method and can be seamlessly integrated into open-vocabulary segmentation methods to tackle the bottlenecks in open-vocabulary segmentation.
By feeding masks and CLIP features into Mask-Adapter, it generates semantic activation maps, which highlight informative regions for each mask. With semantic activation maps, we then gather distinctive information from the CLIP features through pooling to obtain mask embeddings. Then mask embeddings are matched with text embeddings to obtain the classification results. During training, we propose ground-truth mask warmup training and mixed-mask training. At inference, masks generated by the Mask Generator are fed into Mask-Adapter for mask classification.

%\vspace{-8pt} 
\paragraph{Architecture.}
Fig.~\ref{fig:main_arch} illustrates the architecture of Mask-Adapter. Given \( N \) class-agnostic masks \( M_p \), we patchify the binary masks into patches via a simple block comprising two strided \( 3 \times 3 \) convolutional layers, thus generating mask features $\mathcal{F}_{m}$ which have the same resolution as the CLIP features. We then fuse CLIP features $\mathcal{F}_{clip}$  and mask features $\mathcal{F}_{m}$ to obtain the mask region representation $\mathbf{A}_{m} \!=\! \mathcal{F}_{m} + \mathcal{F}_{clip} $. Next, $\mathbf{A}_{m}$ is passed through three ConvNeXt~\cite{liu2022convnet} blocks to enhance the semantics of the mask regions. The refined features are then processed by a final convolutional layer to generate \( K \) semantic activation maps $\mathbf{A}$ for each mask. The semantic activation maps can be expressed as follows:
\begin{equation}
    \mathbf{A} = \text{Conv}(\text{ConvNeXt}^3(\mathbf{A}_{\text{m}}))).
    \label{equ:sam_generate}
\end{equation}
We then obtain the mask embedding \( E_{\text{m}} \) by aggregating information from the CLIP feature maps \( \mathcal{F}_{\text{clip}} \) using the semantic activation maps \( \bar{\mathbf{A}} \), where \( \bar{\mathbf{A}} \) is normalized to 1 for each semantic map. Unlike the mask pooling method, our approach incorporates richer semantic information and includes context beyond the mask region, enhancing the upper bound for open-vocabulary segmentation. The following equation summarizes this process:
\begin{equation}
    E_{\text{m}} = \frac{1}{K} \sum_{k=1}^{K} \bar{\mathbf{A}}_k \cdot \mathcal{F}_{\text{clip}}^T, \quad E_{\text{m}} \in \mathbb{R}^{N \times C}.
    \label{equ:mask_embedding}
\end{equation}
The resulting mask embeddings serve as feature representations for the \( N \) masks, which are then matched with text embeddings to classify the segmentation masks.

\subsection{IoU-based Matcher}
Among the masks generated by the mask generator, multiple masks may correspond to the same object but be misidentified. However, the Hungarian matcher used in previous methods~\cite{stewart2016end,cheng2022masked,carion2020end}, typically finds the optimal match between ground-truth masks and predictions and thus fails to capture these erroneous samples, leading to overfitting in Mask-Adapter training. To address this, we propose an IoU-based matcher that computes the Intersection over Union (IoU) between each ground-truth mask \( y_i \) and predicted mask \( \hat{y}_j \), selecting mask pairs based on a predefined IoU threshold. This approach encourages more diverse training samples than one-to-one matching. The IoU-based matcher is defined as:
\begin{equation}
    \mathcal{M} = \{(i, j) \mid \text{IoU}(y_i, \hat{y}_j) \geq \text{IoU}_{\text{threshold}}\},
    \label{equ:iou_matching}
\end{equation}
where \( \mathcal{M} \) denotes the set of matched pairs. This method enhances classification by incorporating previously misclassified samples, improving the model's robustness.



%\vspace{-8pt}
\subsection{Mask Consistency}

As discussed in~\cite{ge2025alignzeg}, allocating more space in the feature domain for unseen classes improves the recognition of unseen masks. However, directly using a standard classification loss to train the Mask-Adapter can overly crowd the feature space, limiting the model's ability to recognize unseen categories. In contrast to~\cite{ge2025alignzeg}, we adopt a simpler approach by applying a mask consistency loss to mask embeddings of seen class masks.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{sec/figures/fig2.pdf} 
    \vspace{-10pt}
    \caption{\textbf{Mask Consistency Loss.} We compute the cosine loss between the embeddings of the predicted and ground-truth masks to minimize the distance between masks of the same object while leaving a larger feature space for unseen categories.}
    \label{fig:cosine_loss}
    \vspace{-10pt}
\end{figure}
Given the matched predicted and ground-truth masks from the matcher, we feed them into the Mask-Adapter to obtain their respective embeddings \( e^{\text{gt}} \) and \( e^{\text{pred}} \). We then compute the cosine similarity loss between these embeddings as follows:
\begin{equation}
    \mathcal{L}_{\text{cos}}(e^{\text{gt}}, e^{\text{pred}}) = 1 - \sigma_{\cos}(e^{\text{gt}}, e^{\text{pred}}),
\end{equation}
where \( e^{\text{gt}} \) and \( e^{\text{pred}} \) are the embeddings of the ground-truth and predicted masks, respectively, and \( \sigma_{\cos} \) denotes cosine similarity. Mask consistency loss enforces proposal masks with similar IoUs to obtain similar CLIP embeddings, enhancing the recognition of unseen masks and improving the model's robustness, as shown in Fig.~\ref{fig:cosine_loss}.


\subsection{Stable Mask-Text Alignment Training}
To transfer CLIP's open-vocabulary recognition ability with mask-text alignment training is a natural approach for \name{}. However, directly using predicted masks leads to overfitting and training instability. To address it, we propose a two-stage training strategy including ground-truth mask warmup and mixed-mask training.

\paragraph{Ground-truth mask warmup.} We first train the Mask-Adapter using ground-truth masks to avoid low-quality predicted masks, ensuring stable training. This warmup phase enables the Mask-Adapter to develop strong generalization, making it robust to both ground-truth and predicted masks.

\paragraph{Mixed-mask training.} After the warmup training, we mix the predicted masks (from the IoU-based Matcher) and ground-truth masks for training. This mixed-mask training includes low-quality and misclassified masks, enhancing 
\name{}'s robustness and improving its performance on open-vocabulary segmentation tasks.

\paragraph{Overall training loss.} Following~\cite{cheng2022masked,yu2023convolutions}, we use cross-entropy loss for mask classification and cosine loss to enforce mask consistency. The total loss is:

\begin{equation}
    \label{loss}
    \mathcal{L} = \lambda_{ce} \cdot \mathcal{L}_{ce} + \lambda_{cos} \cdot \mathcal{L}_{cos},
\end{equation}
where $\lambda_{ce}$ and $\lambda_{cos}$ are the coefficients for the cross-entropy and cosine losses, respectively.



==> sec/4_experiments.tex <==
\begin{table*}[h!]
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{lllc|cccccc}
        \toprule
        \textbf{Method} & \textbf{VLM} & \textbf{Training Dataset} & & \textbf{A-150} & \textbf{A-847} & \textbf{PC-59} & \textbf{PC-459} & \textbf{PAS-20} \\
        \midrule
        ZegFormer~\cite{ding2022decoupling}  & CLIP ViT-B/16 & COCO-Stuff & & 18.0 & 5.6 & 45.5 & 10.4 & 89.5  \\
        DeOP~\cite{han2023open}  & CLIP ViT-B/16 & COCO-Stuff & & 22.9 & 7.1 & 48.8 & 9.4 & 91.7  \\
        OvSeg~\cite{liang2023open}  & CLIP ViT-B/16 & COCO-Stuff & & 24.8 & 7.1 & 53.3 & 11.0 & 92.6  \\
        SAN~\cite{xu2023san}  & CLIP ViT-B/16 & COCO-Stuff & & 27.5 & 10.1 & 53.8 & 12.6 & 94.0  \\
        OpenSeg~\cite{ghiasi2022scaling}  & ALIGN & COCO Panoptic+Loc. Narr.  & & 28.6 & 8.8 & 48.2 & 12.2 & 72.2  \\
        EBSeg~\cite{shan2024open}  & CLIP ViT-B/16 & COCO-Stuff & & 30.0 & 11.7 & 56.7 & 17.3 & 94.6  \\
        SED~\cite{xie2024sed}  & CLIP ConvNeXt-B & COCO-Stuff & & 31.6 & 11.4 & 57.3 & 18.6 & 94.4  \\
        CAT-Seg~\cite{cho2024cat}  & CLIP ViT-B/16 & COCO-Stuff & & 31.8 & 12.0 & 57.5 & \textbf{19.0} & 94.6  \\
        MAFTP*~\cite{jiao2024collaborative}  & CLIP ConvNeXt-B & COCO-Stuff & & 34.5 & 13.8 & 57.5 & 18.5 & \textbf{95.5} \\
        \rowcolor{gray!10} MAFTP w/ MaskAdapter  & CLIP ConvNeXt-B & COCO-Stuff & & \textbf{35.6} & \textbf{14.2} & \textbf{58.5} & 17.9 & 95.2 \\
        \midrule
        OvSeg~\cite{ghiasi2022scaling}  & CLIP ViT-L/14 & COCO-Stuff & & 29.6 & 9.0 & 55.7 & 12.4 & 94.5  \\
        ODISE~\cite{xu2023open}  & Stable Diffusion & COCO Panoptic & & 29.9 & 11.1 & 55.3 & 14.5 & -  \\
        SAN~\cite{xu2023san}  & CLIP ViT-L/14 & COCO-Stuff & & 32.1 & 12.4 & 57.7 & 15.7 & 94.6  \\
        EBSeg~\cite{shan2024open}  & CLIP ViT-L/14 & COCO-Stuff & & 32.8 & 13.7 & 60.2 & 21.0 & 96.4  \\
        FC-CLIP*~\cite{yu2023convolutions}  & CLIP ConvNeXt-L & COCO Panoptic & & 34.1 & 14.8 & 58.4 & 18.2 & 95.4  \\
        SED~\cite{xie2024sed}  & CLIP ConvNeXt-L & COCO-Stuff & & 35.3 & 13.7 & 60.9 & 22.1 & 96.1  \\
        GBA~\cite{xu2024generalization} & CLIP ConvNeXt-L & COCO Panoptic & & 35.9 & 15.1 & 59.6 & 18.5 & 95.8  \\
        MAFTP*~\cite{jiao2024collaborative} & CLIP ConvNeXt-L & COCO-Stuff & & 36.3 & 15.5 & 59.5 & 21.2 & 96.4  \\
        \rowcolor{gray!10} FC-CLIP w/ MaskAdapter & CLIP ConvNeXt-L & COCO Panoptic & & 36.6 & 14.3 & 59.7 & 19.3 & 95.5 \\
        SMART~\cite{chng2024semantic}  & CLIP ViT-L/14 & COCO Panoptic & & 36.8 & 16.1 & 62.4 & 23.6 & -  \\
        MROVSeg~\cite{zhu2024mrovseg}   & CLIP ViT-L/14 & COCO-Stuff & & 36.9 & 16.1 & \textbf{64.1} & \textbf{24.1} & \textbf{97.6}  \\
        CAT-Seg~\cite{cho2024cat}  & CLIP ViT-L/14 & COCO-Stuff & & 37.9 & 16.0 & 63.3 & 23.8 &  97.0  \\
        \rowcolor{gray!10}MAFTP w/ MaskAdapter  & CLIP ConvNeXt-L & COCO-Stuff & & \textbf{38.1} &  \textbf{16.2} & 60.3 & 22.2 & 95.6  \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Open Vocabulary Semantic Segmentation Performance.} The best results are indicated in bold. We use mIoU as the evaluation metric. * denotes the results re-evaluated.}
\end{table*}

\section{Experiments} 
\label{expr}
In this section, we evaluate the performance of \name{} on open-vocabulary segmentation against the state-of-the-art methods and present detailed ablation studies. Additionally, we explore the potential of integrating \name{} to SAM~\cite{kirillov2023segment} for open-vocabulary segmentation.

\subsection{Experimental Setup} 
\paragraph{Baseline.} To evaluate \name{}, we mainly adopt three baseline methods, \ie, FC-CLIP (\textit{open-vocab.})~\cite{yu2023convolutions}, MAFTP (\textit{open-vocab.})~\cite{jiao2024collaborative}, and Mask2Former (\textit{fixed-vocab.})~\cite{cheng2022masked}.
FC-CLIP and MAFTP utilize mask pooling to extract mask embeddings.
In addition, we follow \cite{ghiasi2022scaling} and adapt the \textit{fixed-vocabulary} Mask2Former to classify masks with mask pooling for a fair comparison.

% For consistency, we used the officially released versions of each model. FC-CLIP and MAFTP are both built upon the ConvNeXt-Large~\cite{liu2022convnet} CLIP backbone from OpenCLIP~\cite{cherti2023reproducible,radford2021learning} and pre-trained on the LAION-2B~\cite{schuhmann2022laion} dataset.

\vspace{-10pt} 

\paragraph{Dataset and evaluation metrics.}
Following the open-vocabulary segmentation setting~\cite{xu2022simple,liang2023open,shan2024open,cho2024cat} and baseline models~\cite{yu2023convolutions,jiao2024collaborative}, we train our Mask-Adapter separately on COCO-Stuff~\cite{caesar2018coco} and on COCO-Panoptic~\cite{lin2014microsoft}. COCO-Stuff consists of 118k images with 171 categories, while COCO-Panoptic has the same training images but contains 133 categories. Notably, training on COCO-Stuff outperforms COCO-Panoptic on open-vocabulary segmentation tasks~\cite{jiao2024collaborative}. We evaluated our model on widely-used open vocabulary segmentation benchmarks, including ADE20K~\cite{zhou2019semantic} (A-847 and A-150), Pascal-Context~\cite{mottaghi2014role} (PC-459 and PC-59), and Pascal-VOC~\cite{everingham2010pascal} (PAS-20). 
Additionally, we assess classification performance on ground-truth masks from ADE20K and explore open-vocabulary segmentation by integrating the Mask-Adapter with the Segment Anything Model~\cite{kirillov2023segment}.

We adopt mean Intersection over Union (mIoU) to evaluate semantic segmentation performance, following~\cite{xu2022simple,liang2023open,shan2024open,cho2024cat,ding2022decoupling}.
To further evaluate the model's generalization ability on unseen categories, we report mIoU\textsuperscript{s} and mIoU\textsuperscript{u} for seen and unseen categories in ablation experiments.

\vspace{-10pt} 

\paragraph{Implementation details.} The proposed \name{} is built on Detectron2~\cite{wu2019detectron2} and trained in two phases. In the first phase, we train \name{} on COCO-Panoptic using ground-truth masks for 20 epochs with a batch size of 8. 
We follow the training schedule~\cite{cheng2022masked,yu2023convolutions} and adopt the AdamW~\cite{loshchilov2017decoupled} optimizer with an initial learning rate of $1 \times 10^{-4}$, weight decay of 0.05, and a multi-step learning rate decay schedule. 
In the second phase, we employ mixed-mask training on COCO-Panoptic for an additional 10 epochs with a batch size of 16. 
All models are trained with random flip and a crop size of 1024$\times$1024, while the evaluation is conducted with an image resolution of 896$\times$896. We set the IoU-based Matcher threshold to 0.7 and $\lambda_{\text{ce}} = 2.0$, $\lambda_{\text{cos}} = 5.0$. The \name{} generates 16 semantic activation maps. Following~\cite{yu2023convolutions}, final classification results are obtained by geometric ensembling in-vocabulary classifiers and Mask-Adapter classification results. The training was conducted on 4 NVIDIA RTX 3090 GPUs.

% lvis + coco panoptic
\begin{table}[h!]
    \centering
    \small
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l|lll}%
        \hline
        \multirow{2}{*}{Method w/o ensemble} & \multicolumn{3}{c}{ADE20K} \\ 
        & mIoU\textsuperscript{s} & mIoU\textsuperscript{u} & mIoU \\ 
        \hline
        Mask2Former w/ CLIP & 34.8 & 17.5 & 26.0 \\
        Mask2Former w/ Ours & 45.3 \textcolor{red}{\scriptsize (+10.5)}  & 21.8 \textcolor{red}{\scriptsize (+4.3)} & 33.4 \textcolor{red}{\scriptsize (+7.4)} \\
        \cdashline{1-4}[1pt/1pt]
        FC-CLIP & 34.6 & 18.6 & 26.5 \\
        FC-CLIP w/ Ours & 46.2  \textcolor{red}{\scriptsize (+11.6)} & 24.8 \textcolor{red}{\scriptsize (+6.2)} & 35.4  \textcolor{red}{\scriptsize (+8.9)} \\
        \cdashline{1-4}[1pt/1pt]
        MAFTP & 45.8 & 27.0 & 36.3 \\
        MAFTP w/ Ours & 46.9  \textcolor{red}{\scriptsize (+1.1)} & 28.6  \textcolor{red}{\scriptsize (+1.6)} & 37.6  \textcolor{red}{\scriptsize (+1.3)} \\
        \hline
    \end{tabular}
    \caption{\textbf{Results of baseline methods on the representative ADE20K dataset.} To more clearly highlight the effectiveness of our approach, we remove the ensemble methods.}
    \label{tab:ablation_woensemble}
    \vspace{-10pt}
\end{table}

\begin{table}[ht]
    \centering
    \small
    \begin{tabular}{l|l|l|cc}
        \toprule
        Model & Source & Mask Embeddings & Acc  \\
        \midrule
        ViT-L/14 & Open CLIP & Mask Cropping & 29.8  \\
        ConvNeXt-L & Open CLIP & Mask Cropping & 40.1  \\
        ViT-L/14 & OVSeg \cite{liang2023open} & Mask Cropping & 49.9 \\
        EVA-L/14\cite{sun2023eva} & EVA-CLIP  & Mask Pooling & 32.2 \\
        EVA-L/14\cite{sun2023eva} & CLIPSelf\cite{wu2023clipself}  & Mask Pooling & 53.1 \\
        ConvNeXt-L & Open CLIP & Mask Pooling & 53.0 \\
        ConvNeXt-L & Open CLIP & \textbf{Mask-Adapter} & 66.7  \\
        ConvNeXt-L & MAFTP & \textbf{Mask-Adapter} & \textbf{74.1}  \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Comparison with different mask embedding extraction methods for classification}. We evaluate previous approaches, including Mask Cropping and Mask Pooling methods.}
    \label{tab:ablation_mask_adapter}
    \vspace{-10pt}
\end{table}


\subsection{Main Results}
\paragraph{Open-vocabulary segmentation.} We follow standard settings~\cite{cho2024cat,xu2023san,jiao2024collaborative} to evaluate open-vocabulary segmentation. We classify the models based on the size of the Vision-Language Model (VLM). For base VLM models, Our Mask-Adapter combined with MAFTP~\cite{jiao2024collaborative} achieves the best performance on the A-150, A-847, and PC-59 datasets, with mIoU scores of 35.6, 14.2, and 58.5, respectively, improving mIoU by 1.1, 0.4, and 1.0 compared to the baseline. For large VLMs, our Mask-Adapter with MAFTP outperforms the state-of-the-art method, CAT-Seg~\cite{cho2024cat}, achieving the best results on the challenging A-150 and A-847 datasets. Compared to the baseline FC-CLIP~\cite{yu2023convolutions}, our approach improves mIoU by 2.5, 1.3, and 1.1 on the A-150, PC-59, and PC-459 datasets, respectively, demonstrating its effectiveness. Moreover, compared to the baseline MAFTP~\cite{jiao2024collaborative}, our approach improves mIoU by 1.8, 0.7, 0.8, and 1.0 on the A-150, A-847, PC-59, and PC-459 datasets, respectively, proving the adaptability of our method, which can be seamlessly integrated into open-vocabulary segmentation frameworks based on mask pooling in a plug-and-play manner.






\paragraph{Comparisons on ADE20K without ensemble strategy.}
To demonstrate the Mask-Adapter's effectiveness, we conduct experiments on ADE20K without the ensemble strategy. As shown in Tab.~\ref{tab:ablation_woensemble}, incorporating Mask-Adapter significantly boosts the performance of three baselines: Mask2Former (+28.4\%), FC-CLIP (+33.5\%), and MAFTP (+3.6\%), highlighting the substantial improvements in open-vocabulary segmentation.




\begin{table}[ht]
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{cccc|ccc}
        \toprule
        \multirow{2}{*}{GT.} & \multirow{2}{*}{Pred.} &  \multirow{2}{*}{Warmup} &\multirow{2}{*}{Mask Cons.}  & \multicolumn{3}{c}{ADE20K} \\ 
        & & & & mIoU\textsuperscript{s} & mIoU\textsuperscript{u} & mIoU \\
        \midrule
         &  &  &  & 34.6 & 18.6 & 26.5 \\
         \checkmark&  &  & & 44.7 & 23.9 & 34.1 \\
         %& \checkmark &  &  &47.8 & 24.4 & 35.9 \\
         \checkmark& \checkmark &  & & 45.4 & 23.3 & 34.3 \\
         \checkmark& \checkmark & \checkmark & & 45.6 & 23.8 & 34.6 \\
         \checkmark& \checkmark & \checkmark &\checkmark &\textbf{46.2} & \textbf{24.8} & \textbf{35.4} \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Ablation study of Mask-Adapter training strategies and methods.} GT. refers to ADE20K ground truth masks, Pred. denotes FC-CLIP predicted masks, Mask Cons. indicates whether mask consistency is applied, and GT Warmup refers to the warmup using ground truth masks. We remove the ensemble operation here.}
    \label{tab:ablation_mask_adapter_training}
    \vspace{-10pt}
\end{table}




\paragraph{Comparisons with Zero-shot Mask Classification Methods.}
Tab.~\ref{tab:ablation_mask_adapter} presents results of various zero-shot mask classification methods on the ADE20K dataset using ground-truth masks. Our method achieves 74.1\% accuracy, outperforming the methods in \cite{xu2022simple,ding2022decoupling,liang2023open,jiao2024collaborative,yu2023convolutions} demonstrating the effectiveness of our Mask-Adapter in transferring CLIP's open-vocabulary recognition capabilities to mask classification.



\subsection{Ablation Study}


\paragraph{Ablation of Mask-Adapter.}
As shown in Tab.~\ref{tab:ablation_mask_adapter_training}, replacing Mask Pooling with the ground-truth trained Mask-Adapter in FC-CLIP improves mIoU by 10.1 and 5.3 for seen and unseen categories, respectively. However, directly using mixed predicted and ground-truth masks for training slightly reduces performance on unseen classes. Introducing Ground-truth warmup and mask consistency loss improves mIoU by 0.3 and 0.8, respectively, highlighting the importance of Mask Consistency and Ground-Truth Warmup in enhancing the model's robustness.

\begin{table}[ht]
    \centering
    \small
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l|c|ccc}
        \toprule
         &  & \multicolumn{3}{c}{ADE20K} \\
        Matcher& Threshold & mIoU\textsuperscript{s} & mIoU\textsuperscript{u} & mIoU \\
        \midrule
        Hungarian  & - & 47.4 & 24.6 & 35.9 \\
        IoU-based  & 0.7 & \textbf{47.8} & \textbf{25.0} & \textbf{36.2}  \\
        IoU-based  & 0.8 & 47.2 & 24.7 & 35.8 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Ablation study of different matchers and IoU thresholds.}We evaluate the impact of various matchers and IoU thresholds on ADE20K dataset.}
    % We evaluate the impact of various matchers and IoU thresholds on ADE20K dataset.}

    \label{tab:ablation_matcher}
    \vspace{-10pt}
\end{table}

% \begin{table}[ht]
%     \centering
%     \footnotesize
%     \begin{tabular}{cccc|ccc}
%         \toprule
%         \multirow{2}{*}{GT.} & \multirow{2}{*}{Pred.} & \multirow{2}{*}{Mask Cons.} & \multirow{2}{*}{GT Warmup} & \multicolumn{3}{c}{ADE20K} \\ 
%         & & & & mIoU\textsuperscript{s} & mIoU\textsuperscript{u} & mIoU \\
%         \midrule
%          &  &  &  & 34.6 & 18.6 & 26.5 \\
%          \checkmark&  &  & & 47.3 & 23.9 & 35.4 \\
%          & \checkmark &  &  &47.8 & 24.4 & 35.9 \\
%          \checkmark& \checkmark &  & & 48.0 & 24.0 & 35.8 \\
%          \checkmark& \checkmark & \checkmark & & 48.5 & 24.4 & 36.3 \\
%          \checkmark& \checkmark & \checkmark &\checkmark &\textbf{48.0} & \textbf{25.5} & \textbf{36.6} \\
%         \bottomrule
%     \end{tabular}
%     \caption{\textbf{Ablation study of Mask-Adapter training strategies and components.} GT. refers to ADE20K ground truth masks, Pred. denotes FC-CLIP predicted masks, Mask Cons. indicates whether mask consistency is applied, and GT Warmup refers to the warmup using ground truth masks.}
%     \vspace{-10pt}
% \end{table}







\begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.95\linewidth]{sec/figures/vis_semanticmap.pdf}
    \vspace{-5pt}
    \caption{\textbf{Visualizations for Semantic Activation Maps.} We present the visualizations of the semantic activation maps and segmentation masks. For each input image, the upper row shows the semantic activation maps and the bottom row shows the corresponding segmentation masks. The semantic activation maps tend to highlight the discriminative regions of the mask.
    Best viewed on screen after zooming in.}
    \label{fig:vis_sam_mask}
    \vspace{-5pt}
\end{figure*}

\paragraph{Ablation study of different matchers and IoU thresholds.} 
As shown in Tab.~\ref{tab:ablation_matcher}, we evaluate the impact of different matchers on the ADE20K dataset. The IoU-based matcher outperforms the Hungarian matcher in terms of mIoU for unseen classes. With an IoU-based matcher threshold of 0.7, the model improves by 0.3 mIoU overall, and 0.4 mIoU for seen and unseen classes.


\begin{table}[ht]
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    \scalebox{1.0}{
    \begin{tabular}{l|c|c|c}
        \toprule
         &\centering Patch Embedding & GT mIoU & FC-CLIP mIoU  \\
        \midrule
        \multirow{3}{*}{\centering (a)} 
        & Concat & 42.5 & 35.2 \\
        & Add + $2 \times 3 \times 3$ Conv  & \textbf{43.4} & \textbf{35.4} \\
        & Add + $4 \times 4$ Conv & \textbf{43.4} & 35.2 \\
        \midrule
        & \centering Num Blocks  & GT mIoU & FC-CLIP mIoU \\
        \midrule
        \multirow{3}{*}{\centering (b)} 
        & 2 &  43.1 & \textbf{35.4} \\
        & 3 & 43.4 & \textbf{35.4} \\
        & 4 & \textbf{43.7} & 35.3 \\
        \midrule
        & \centering CLIP Feature  & GT mIoU & FC-CLIP mIoU \\
        \midrule
        \multirow{2}{*}{\centering (c)} 
        & with  & \textbf{43.4} & \textbf{35.4} \\
        & w/o  & 35.5 & 32.5 \\
        \bottomrule
    \end{tabular}}
    \caption{\textbf{Ablation study on different designs in Mask-Adapter}, analyzing the impact of different patch embedding methods, ConvNeXt block counts, and input CLIP feature usage. Section (a) compares patch embedding strategies, (b) examines the effect of varying ConvNeXt block numbers, and (c) highlights the importance of including CLIP features.}
    \label{tab:patch_embedding_cnext_clip_feature}
\end{table}





\vspace{-6pt} 

\paragraph{Ablation study on different designs in Mask-Adapter.}
Tab.~\ref{tab:patch_embedding_cnext_clip_feature} presents an ablation study on key Mask-Adapter design choices. In (a), we show that integrating mask embeddings with CLIP features outperforms simple concatenation, proving this fusion strategy is the most effective. Our mask patchify approach, with two 3$\times$3 convolutions, outperforms a single 4$\times$4 convolution. In (b), we find that increasing ConvNeXt block count improves mask classification accuracy with ground-truth masks, but too many blocks cause overfitting. Three blocks strike the optimal balance. In (c), incorporating CLIP features significantly improves both Mask Accuracy and mIoU, enhancing semantic representation.












% \begin{table}[ht]
%     \centering
%     \small
%     \renewcommand\tabcolsep{3.5pt}
%     \renewcommand\arraystretch{1.1}
%     \scalebox{0.90}{
%     \begin{tabular}{l|c|c|c|ccc}
%         \toprule
%         \multirow{2}{*}{Matcher} & \multirow{2}{*}{Cos Loss} & IoU & Cos & \multicolumn{3}{c}{ADE20K} \\ 
%         & & Th. & W. & mIoU\textsuperscript{s} & mIoU\textsuperscript{u} & mIoU \\
%         \midrule
%         Hungarian Matcher &  & - & 10.0 & 47.4 & 24.8 & 36.0 \\
%         \midrule
%         IoU Matcher &  & 0.8 & 0.0 & 47.2 & 24.7 & 35.8 \\
%         \midrule
%         IoU Matcher &  & 0.7 & 0.0 & 47.8 & 25.0 & 36.2 \\
%         IoU Matcher & √ & 0.7 & 2.0 & 47.8 & 24.7 & 36.1 \\
%         IoU Matcher & √ & 0.7 & 5.0 & \textbf{48.0} & \textbf{25.5} & \textbf{36.6} \\
%         IoU Matcher & √ & 0.7 & 10.0 & 47.4 & 24.8 & 36.0 \\
%         \bottomrule
%     \end{tabular}}
%     \caption{\textbf{Ablation study of different Matcher configurations, Cosine Loss usage, IoU Thresholds, and Cosine Loss Weights in Mask Consistency.} Open vocabulary segmentation performance is evaluated on the ADE20K dataset. For `IoU Matcher`, the best results are achieved with an IoU threshold of 0.7 and cosine loss weight of 5.}
%     \label{tab:ablation_combined}
%     \vspace{-10pt}
% \end{table}
\paragraph{Ablation of ground-truth masks warmup datasets.}
Tab.~\ref{tab:ablation_gt_training_data} evaluates the impact of different dataset combinations for Ground-truth masks warmup training in open-vocabulary segmentation. While COCO-Panoptic is a standard choice, we observed overfitting with this dataset, leading to reduced accuracy for unseen categories over time. To address this, we incorporate additional datasets. LVIS enhances Mask-Adapter’s robustness, likely due to its richer textual information. However, integrating a subset of the Grand dataset~\cite{rasheed2024glamm} (2\% of the SA-1B \cite{kirillov2023segment}) led to performance degradation compared to the COCO-only baseline, likely due to mask quality problems.

\begin{table}[h]
    \centering
    \small
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l|cc}
        \toprule
        Datasets & GT mIoU & FC-CLIP mIoU \\
        \midrule
        COCO-P & 43.4 & 35.4 \\
        COCO-P, LVIS & \textbf{44.5} & \textbf{36.4} \\
        COCO-P, LVIS, Grand & 43.6 & 35.1 \\
        % COCO-P, LVIS, O365 (Mask) & 42.0 & 34.8 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Ablations on Ground Truth Training Data.} Comparison of open-vocabulary segmentation performance (mIoU) on ADE20K, utilizing Ground Truth masks and FC-CLIP predicted masks under different dataset combinations.}
    \label{tab:ablation_gt_training_data}
\end{table}

\begin{table}[ht]
    \centering
    \small
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l|cccc}
        \toprule
         & A-847 & A-150 & PC-459 & PC-59 \\
        \midrule
        SAM w/ CLIP & 7.1 & 17.9 & 6.4 & 34.4 \\
        SAM w/ MAFT & 10.1 & 29.1 & 12.8 & \textbf{53.5} \\
        SAM w/ Mask-Adapter & \textbf{11.4} & \textbf{31.5} & \textbf{16.8} & 49.5 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Comparison of SAM and SAM with Mask-Adapter under open-vocabulary settings.} Following~\cite{jiao2023learning}, we evaluate performance using SAM-H with a standard CLIP model and MAFT~\cite{jiao2023learning}, as well as our Mask-Adapter approach.} 
    \label{tab:comparison_sam}
\end{table}





% \begin{table}[h]
%     \centering
%     \small
%     \begin{tabular}{l|cc}
%         \toprule
%         Datasets & GT mIoU & FC-CLIP mIoU \\
%         \midrule
%         COCO-P & 43.4 & 35.4 \\
%         COCO-P, LVIS & \textbf{44.5} & \textbf{36.4} \\
%         COCO-P, LVIS, Grand & 43.6 & 35.1 \\
%         COCO-P, LVIS, O365 (Mask) & 42.0 & 34.8 \\
%         \bottomrule
%     \end{tabular}
%     \caption{\textbf{Ablations on Ground Truth Training Data.} Comparison of open-vocabulary segmentation performance (mIoU) on ADE20K, utilizing Ground Truth masks and FC-CLIP predicted masks under different dataset combinations.}
%     \label{tab:ablation_gt_training_data}
% \end{table}






\subsection{Segment Anything with Mask-Adapter}
Mask-Adapter can be seamlessly integrated into SAM without training, significantly enhancing its performance in open-vocabulary segmentation tasks. Following \cite{jiao2023learning}, we conduct experiments under \textit{open-vocabulary settings}. Tab. \ref{tab:comparison_sam} shows that SAM with the Mask-Adapter outperforms SAM w/ CLIP or w/ MAFT across multiple datasets, highlighting the Mask-Adapter's effectiveness in improving the classification accuracy of masks generated by SAM.


==> sec/5_conclusion.tex <==
\section{Conclusion}
In this work, we reveal severe limitations of prevalent methods using mask pooling and predicted masks for open-vocabulary segmentation and present a simple yet effective \name{}.
Instead of directly using proposal masks, \name{} extracts semantic activation maps from masks and obtains mask embedding by aggregating CLIP features according to the semantic and contextual information provided by the semantic activation maps for mask classification. We integrate \name{} into several well-established open-vocabulary segmentation methods, demonstrating significant performance gains and achieving state-of-the-art results across multiple datasets. \name{} also extends to SAM without training and achieves impressive results on several open-vocabulary segmentation benchmarks.


==> sec/_1_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

